Long-term scintillation studies of EPTA pulsars. I. Observations and basic results

Interstellar scintillation analysis of pulsars allows us to probe the small-scale distribution and inhomogeneities of the ionized interstellar medium. Our priority is to present the data set and the basic measurements of scintillation parameters of pulsars employing long-term scintillation observations carried out from 2011 January to 2020 August by the European Pulsar Timing Array radio telescopes in the 21-cm and 11-cm bands. Additionally, we aim to identify future possible lines of study using this long-term scintillation dataset. We present the long-term time series of $\nu_{\rm d}$ and $\tau_{\rm d}$ for 13 pulsars. Sanity-checks and comparisons indicate that the scintillation parameters of our work and previously published works are mostly consistent. For two pulsars, PSRs~J1857+0943 and J1939+2134, we were able to obtain measurements of the $\nu_{\rm d}$ at both bands, which allows us to derive the time series of frequency scaling indices with a mean and a standard deviation of 2.82$\pm$1.95 and 3.18$\pm$0.60, respectively. We found some interesting features which will be studied in more detail in subsequent papers in this series: (i) in the time series of PSR~J1939+2134, where the scintillation bandwidth sharply increases or decreases associated with a sharp change of dispersion measure; (ii) PSR~J0613$-$0200 and PSR~J0636+5126 show a strong annual variation in the time series of the $\tau_{\rm d}$; (iii) PSR~J1939+2134 shows a weak anti-correlation between scintillation timescale and dispersion in WSRT data.

==> README <==
This directory contains the pulsar BibTeX database and various associated
files. 

Files include:
    Journal databases: journals.bib and journals_apj.bib have macros for
       journal names as long abbreviations and short ApJ abbreviations,
       respectively.

    Pulsar databases:
       psrrefs.bib.  The main pulsar database, kept READ ONLY.  It will be
           updated occasionally (roughly annually), from the contents
           of modrefs.bib.
       modrefs.bib.  This contains modified items or additions to the
           database.  To modify an item, the entry in psrrefs.bib should
           be copied into modrefs.bib and edited appropriately, with an
           explanatory message in the `crtr' field.  To add a
           new item, use a unique key as described below.
       crossrefs.bib.  This file contains conference proceedings entries
           that are cross referenced in modrefs and psrrefs.  These must
           be included LAST for BibTeX to properly resolve cross references.

       To use the pulsar databases, your LaTeX file should contain the command:
           \bibliography{journals_apj,modrefs,psrrefs,crossrefs}  
           (N.B. the argument order is important).

    Gamma-ray burst database: grbrefs.bib.  Modifications and
           additions can be made directly to this file (there is no
           "modrefs" file).  Cross references should be added AT THE END
           OF THE FILE, not in alphabetical order.

       To use the GRB database, your LaTeX file should contain the command:
           \bibliography{journals_apj,grbrefs}

       The pulsar and GRB databases can be used together, although care is
           needed because of duplicated tags.  Please avoid duplicate tags
           in the future. 

    Helpful hint:
       To minimize the garbage that BibTeX produces with duplicate
       entries (which you will have if you have modifications), it is
       recommended that you use the following alias for bibtex:
  alias bibtex 'bibtex \!:1 | grep -v skipp | grep -v "," | grep -v message'

---------------------------------------------------------------------------

In all of the BibTeX databases, the following rules should be
adhered to:

              RULES FOR MAINTAINING THE PULSAR BibTeX DATABASE


1. Keep the entries sorted in alphabetical order, by key if possible.

2. Make all references to journals symbolic. Look in the JOURNALS.BIB file
   for a list of the abbreviations, and add further ones if necessary.  

3. In an attempt to keep the keys unique use the following rules

	a. Single author: use three letters, such as lyn82 for Lyne 1982.
	b. Two--four authors: use first letter of authors' surnames, as
	   in lmt85 for Lyne, Manchester, & Taylor 1985.
	c. More than four authors: use first letters of first three
	   authors' surnames, followed by +, as in hbp+68 for Hewish
	   et al, 1968.
	d. To break ties, use a letter after the year, as in ht75a, ht75b.
        e. For multi-word surnames: use the first letter of the first word,
           eg "v", not "h" for "van den Heuvel."  

4. Follow the general layout of the entries currently used, i.e. put each
   field on a new line as it makes it much easier to read.
   Always include a title.  Note that for conference proceedings and
   the like, please define the book as a reference (in crossrefs.bib).
   Subsequent entries can then cross reference the book. For an example,
   see jwb96 (book) and rlg96 (article). This method reduces the overheads
   on future updates, uniforms book definitions, and minimizes typos.

5. When making an entry in modrefs to correct an error in psrrefs, please
   add a line
   ,crct={spell} (or page, volume, etc)
   to assist the poor soul who is next to merge the files.

6. If an entry should be deleted, insert a line as follows in the entry.
   ,deleteme=1
   Do NOT delete the entry.  It will be deleted at the next collation.

7. Please try to avoid duplicating tags not only within a file but across all
   files in this directory.  (So if mt77 is used in psrrefs.bib, don't
   use it in grbrefs.bib -- use mt77b, etc.)  Use the supplied checkref
   utility before adding new entries.

   If these rules are adhered to then a useful database can be slowly built
   up as more people add to it.

  Paul Harrison, 
  revised by J. H. Taylor 1991, 
  V. M. Kaspi and S. E. Thorsett 1999.
  Rule 3e (which, admittedly, contravenes some conventions; sorry!) 
       added by I. H. Stairs 2011 

-------------------------------------------------------------------


Other useful things in this directory:

checkref: a shell script to search through the entries of all BibTeX file
          in this directory.  Set PSRREFS environment variable to point
          to this directory before using.

merge.pl: a perl script (that uses the Text::BibTeX module*)
          that will merge bibliography files, sort the result, and identify
          duplicate entries.

	  Note: to use this file, checkout and install the btparse and
          BibTeX modules from the CVS archive (just like you checked out
          psrrefs).  These are slightly modified from the production
          versions (to eliminate warning messages for names with embedded
          \" characters).  Using the production version of Text::BibTeX
          will also work.

listall:  a shell script to provide a latex listing of all the entries in 
          psrrefs, permitting a check for syntax and other errors.  Due to 
          the limited capacity of TeX buffers, the database has to be split 
          into three segments, each limited to about 1900 entries.  This 
          script will fail when the database exceeds about 5700 keys.

          Note: to use this, you will need to checkout listall.tex and 
          listall.bst.  For debugging the database, you may find it useful 
          to study the files listall1.blg, listall2.blg and listall3.blg.

------------------------------------------------------------

          CREDITS

This database was built through the hard work of many people (so be
gentle with it!).  Sites contributing to the pulsar databases include:
   Amsterdam  (Ben Stappers)
   Arecibo (Paulo Freire)
   ATNF  (Dick Manchester, Simon Johnston)
   NAO-Beijing (Jinlin Han)
   Harvard (Bryan Gaensler)
   Jodrell Bank  (Andrew Lyne, Michael Kramer) 
   McGill (Vicky Kaspi)
   Bryn Mawr (David Nice)
   UBC (Ingrid Stairs)
   UCSC  (Steve Thorsett)

Additional sites contributing to the GRB database include
   Caltech (Fiona Harrison)
   STScI (Andy Fruchter)

Database merging has been done by several people over the years, major ones 
most recently by Vicky Kaspi (Nov 1999), Paulo Freire and Andrew Lyne 
(Jan 2003), Dick Manchester (Dec 2005) and Ingrid Stairs (Feb. 2008).









==> checkref <==
#!/bin/sh
# Set your environment variable PSRREFS to point to the directory where
# you keep your BibTeX databases
# I use gnu awk.  Your mileage may vary with other awks.
# No warranties!  --Steve Thorsett

args="$(echo $@ | sed 's/,/ /g')"

for reference in $args
do
  search=`echo $reference | sed -e 's/\+/\\\+/'`
  (for file in $PSRREFS/psrrefs.bib $PSRREFS/modrefs.bib $PSRREFS/crossrefs.bib $PSRREFS/grbrefs.bib; 
do cat $file | 
  grep -v ^% | 
  gawk 'BEGIN         {IGNORECASE=1; RS=""; ORS="\n\n"} 
  /'"$search"'/ {print " ====> From: '"$file"' <===="; print $0}';
done ) | less
done


==> listall <==
grep @ psrrefs.bib | awk -F\{ '{print $2}' | awk -F, '{print "\\nocite{"$1"}"'} > allkeys.tex

head -1900 allkeys.tex > keys1.tex
tail +1901 allkeys.tex | head -1900 > keys2.tex
tail +3801 allkeys.tex > keys3.tex

rm listall.aux
rm listall.bbl
cp keys1.tex keys.tex
latex listall
bibtex listall
latex listall
latex listall
mv listall.blg listall1.blg
mv listall.dvi listall1.dvi
mv listall.log listall1.log
dvips listall1

rm listall.aux
rm listall.bbl
cp keys2.tex keys.tex
latex listall
bibtex listall
latex listall
latex listall
mv listall.blg listall2.blg
mv listall.dvi listall2.dvi
mv listall.log listall2.log
dvips listall2

rm listall.aux
rm listall.bbl
cp keys3.tex keys.tex
latex listall
bibtex listall
latex listall
latex listall
mv listall.blg listall3.blg
mv listall.dvi listall3.dvi
mv listall.log listall3.log
dvips listall3



